Simple, Light, Yet Formally Verified, Global Common Subexpression Elimination and Loop-Invariant Code Motion

We present an approach for implementing a formally certified loop-invariant code motion optimization by composing an unrolling pass and a formally certified yet efficient global subexpression elimination.This approach is lightweight: each pass comes with a simple and independent proof of correctness.Experiments show the approach significantly narrows the performance gap between the CompCert certified compiler and state-of-the-art optimizing compilers.Our static analysis employs an efficient yet verified hashed set structure, resulting in fast compilation.

==> benchmark_data/measures_kvx_simulator.tex <==
glpk & 1.00 & 1.00 & 0.99 & 0.98 & 1.01 & 0.95\\
picosat & 1.00 & 1.00 & 1.00 & 0.99 & 1.00 & 0.97\\
genann4 & 0.98 & 0.98 & 0.84 & 0.88 & 1.05 & 0.65\\
jpeg-6b & 1.01 & 1.00 & 0.99 & 0.97 & 1.09 & 0.92\\
ocaml & 1.03 & 0.98 & 1.00 & 1.02 & 1.10 & 1.06\\
\hline
correlation & 0.97 & 0.99 & 0.99 & 0.99 & 0.53 & 0.50\\
covariance & 0.91 & 0.98 & 0.90 & 0.97 & 0.95 & 0.73\\
2mm & 0.92 & 0.83 & 0.77 & 0.83 & 1.01 & 0.75\\
3mm & 0.91 & 0.97 & 0.85 & 0.88 & 1.05 & 0.76\\
atax & 0.91 & 0.90 & 0.85 & 0.84 & 1.12 & 0.84\\
bicg & 0.94 & 1.03 & 0.93 & 0.93 & 1.18 & 0.93\\
cholesky & 0.91 & 0.95 & 0.83 & 0.83 & 1.02 & 0.79\\
doitgen & 0.87 & 0.83 & 0.92 & 0.86 & 0.84 & 0.55\\
gemm & 0.96 & 0.92 & 0.87 & 0.95 & 1.09 & 0.91\\
gemver & 0.99 & 0.99 & 0.89 & 0.93 & 1.22 & 0.90\\
gesummv & 0.97 & 0.97 & 0.91 & 0.96 & 1.12 & 0.93\\
mvt & 0.93 & 0.93 & 0.92 & 0.94 & 1.12 & 0.81\\
symm & 1.03 & 1.02 & 1.01 & 1.01 & 1.08 & 0.82\\
syr2k & 1.02 & 1.02 & 1.00 & 1.02 & 1.12 & 0.86\\
syrk & 0.96 & 0.96 & 0.75 & 0.79 & 1.04 & 0.68\\
trisolv & 0.93 & 0.93 & 0.78 & 0.81 & 1.06 & 0.80\\
trmm & 1.00 & 1.04 & 0.80 & 0.81 & 1.03 & 0.82\\
durbin & 0.93 & 0.91 & 0.87 & 0.87 & 1.13 & 0.77\\
dynprog & 0.92 & 0.89 & 0.93 & 0.81 & 1.30 & 0.84\\
gramschmidt & 0.97 & 0.90 & 0.91 & 0.87 & 1.02 & 0.80\\
lu & 1.08 & 1.08 & 0.86 & 0.90 & 1.06 & 0.92\\
ludcmp & 0.95 & 0.94 & 0.84 & 0.81 & 0.91 & 0.74\\
floyd-warshall & 1.00 & 1.04 & 1.00 & 1.00 & 0.78 & 0.91\\
reg\_detect & 0.88 & 0.86 & 0.71 & 0.68 & 0.75 & 0.60\\
adi & 0.99 & 0.99 & 0.99 & 0.99 & 0.99 & 0.99\\
fdtd-2d & 0.94 & 0.97 & 0.85 & 0.86 & 0.93 & 0.81\\
jacobi-1d-imper & 1.00 & 1.00 & 0.89 & 0.86 & 1.09 & 0.92\\
jacobi-2d-imper & 0.98 & 0.98 & 0.94 & 0.95 & 0.97 & 0.80\\
seidel-2d & 1.00 & 1.00 & 1.00 & 1.00 & 1.02 & 0.99\\

